Publishing Efficient On-device Models Increases Adversarial Vulnerability

Recent increases in the computational demands of deep neural networks (DNNs) have sparked interest in efficient deep learning mechanisms, e.g., quantization or pruning. These mechanisms enable the construction of a small, efficient version of commercial-scale models with comparable accuracy, accelerating their deployment to resource-constrained devices. In this paper, we study the security considerations of publishing on-device variants of large-scale models. We first show that an adversary can exploit on-device models to make attacking the large models easier. In evaluations across 19 DNNs, by exploiting the published on-device models as a transfer prior, the adversarial vulnerability of the original commercial-scale models increases by up to 100x. We then show that the vulnerability increases as the similarity between a full-scale and its efficient model increase. Based on the insights, we propose a defense, $similarity$-$unpairing$, that fine-tunes on-device models with the objective of reducing the similarity. We evaluated our defense on all the 19 DNNs and found that it reduces the transferability up to 90% and the number of queries required by a factor of 10-100x. Our results suggest that further research is needed on the security (or even privacy) threats caused by publishing those efficient siblings.

==> contents/note.tex <==

[Discussion at the point] \\
> server-side model and client-models \\
> adversarial examples \\
> client, server, adversarial examples \\

[V. Similarity... Results] \\
> trivial solutions, if we release a new model than it's fine... (Section III-C) \\
> Input-gradients, making it explicit... \\
> $f_server, f_client$ | client, on-device (fix the notations: $f_s$, $f_c$, remove edge) \\
> Figure <the reason to run this figure>, \\
 >> what to think about the figure... (what it is in the context) \\

[VI. Evaluation]
> Not push everything into the evaluations.... \\
>> A person to wait it not good \\
>> (0.1 - doesn't work for three, split this into two figures) \\
>> Separate section, to talk about the feature-level similarity doesn't work... \\



[Appendix] \\
To-do list \\
1. Discuss ineffective feature-level similarity measures \\
2. Discuss ineffective re-training models with our loss from scratch \\
3. Explain our training details \\
4. 

==> contents/old.tex <==

% Copy the rest of introduction starting from "We  begin  by  conducting  a  comprehensive  analysis..." paragraph.



\section{Introduction}
\label{sec:intro}

% ----------------------------------------------------------------
%   DNNs are becoming computationally expensive
% ----------------------------------------------------------------
%
Deep neural networks (DNNs) enable many tasks that were previously seen as intractable, such as self-driving cars with object recognition models~\cite{Wang:CVPR19} or writing human-like texts~\cite{Brown:NIPS20}.
%
In order to achieve these %goals 
advancements, one of the most important factors
is their \emph{scale}.
% 
Compared to the 61 million parameter AlexNet model~\cite{AlexNet} from a decade ago, 
current state-of-the-art classifiers have
over 15 billion parameters ($246\times$ larger) \cite{ruiz2021scaling}.
%EfficientNets~\cite{EfficientNet, EfficientNetL2}, uses 8$\times$ more parameters ($\sim$480 millions).
% 
In the domain of neural language models,
the largest models exceed one trillion parameters~\cite{Fedus:arXiv2011}.

% \added{
% Motivation for research in general:

% 1. Models are getting pushed on device (references to Apple CSAM, Google on device spam, etc...).
% 2. Some of the tasks for on-device models have counterparts in other product or in the cloud (for sure Apple run CSAM on Apple Cloud)
% 3. On-device model sufficiently easy to reverse engineer and attack
% 4. Our research question: does this help attacking models in other products/cloud? what can we do to remediate it?

% Motivation for specific experiments:

% We can expect that if a company have on-device and cloud model then they may be trained on the same data, using similar architectures, using distillation, ...}



% ----------------------------------------------------------------
%   Efficient deep learning is proposed to solve this issue
% ----------------------------------------------------------------
%
DNNs of this %size 
scale %necessarily 
require specialized environments to run.
%
OpenAI's 175 billion parameter GPT-3 model is only available through a query interface in part
because %of the fact that 
it is technically infeasible to run inference on a single machine.
% 
\begin{comment}
    Pushing %larger and 
    larger models to servers does have other drawbacks.
    %
    Paramount among these is the fact that users may be reluctant to share
    their personal information with remotely hosted models.
    %
    For example, Apple recently announced that all images uploaded to
    their servers would be scanned for child abuse material~\cite{AppleCS}.
    %
    However, 
    while more accurate,
    running this inference on the server would violate the privacy of users who must now reveal their plaintext images to Apple.
    % This would be [bad]
\end{comment}
%
To remedy this issue, 
recent work in efficient deep learning develops methods that create smaller, more efficient on-device variants of %server-side 
the original models with a comparable accuracy.
%
These methods range from the classical model-compression~\cite{FirstQuantization, Pruning, NASNet, MobileNet, SqueezeNet} to more sophisticated ones~\cite{ProxylessNAS, AutoMLforEDL, OFA}.
% 
\begin{comment}
    Continuing on the above example, Apple decided to deploy an on-device model that initially performs this abuse detection before upload.
    %
    Images will only be uploaded to the remote model for further classification %and human review 
    if the on-device models flag the content as suspicious (or malicious).%, at which point more powerful server-side on-device models can perform classification for further inspection.
\end{comment}


% ----------------------------------------------------------------
%   No security concerns are there for those models
% ----------------------------------------------------------------
% 
However, this practice of releasing on-device models raises a new interesting \emph{security} question. % not considered in prior work.
%
Recent work has shown the vulnerability of DNNs to \emph{adversarial examples}~\cite{Intriguing, PGD, FGSM, CNW, AutoZoom, P-RGF, BanditsTD, BanditsNPrior, Evasion, PapernotLimits, DeepFool, HybridBatch, DRMI}, where an adversary can make small perturbations to inputs so that the model makes controlled mistakes.
%
% For example, an adversary can imperceptibly modify an image that is supposed to be detected as abusive such that it is detected as benign content by a model but still looks visually identical to humans.
For example, an adversary can imperceptibly modify a legitimate user's image such that it is detected as abusive by %both on-device and server-side models 
any models (similar to a DoS attack on the user).
%
Fortunately, when only query access is allowed, crafting successful adversarial examples on models typically requires thousands of queries~\cite{DecisionBased,HopSkipJump}.
%
%The widespread adoption of efficient deep learning in many real-world applications, \textit{e.g.}, smart home, smart cars, or smart healthcare~\cite{SmartHome:MobiSys18, SmartHealthcare:FGCS20, SmartCar:DIVANet21}, calls for an understanding of its security implications.



% Incorporated into the previous section, but saved for later
\begin{comment}
    Independent of any of the above,
    recent work has shown the vulnerability of machine
    learning models to \emph{adversarial examples} [cites],
    where an adversary can make small perturbations to
    machine learning inputs so that the model makes controlled mistakes.
    %
    For example, an adversary can imperceptibly modify an image that is supposed to 
    be detected as abusive so that instead it is detected as benign content
    by a machine learning model but still looks visually identical to humans.
\end{comment}



% ----------------------------------------------------------------
%   Briefly introduce the research question we will explore
% ----------------------------------------------------------------
%
In this paper, we study the security considerations of releasing 
smaller on-device variants of % large remote 
large-scale models 
obtained by efficient deep learning techniques.
%
Specifically, we ask the following questions:
%
\begin{quote}
    \emph{How much more vulnerable are %server-side 
    the original models when
    on-device models are released?
    Is there a release strategy that does not increase vulnerability?}
\end{quote}
%
We focus on this question in particular to understand the broader question
of how releasing on-device models impacts security and privacy generally.


==> figures/defense/defense_summary.tex <==


% [Figure] defense summary
\begin{figure*}[t]
\centering
% 
\minipage{0.49\textwidth}
  \includegraphics[width=\linewidth]{figures/defense/defense_transfer.pdf}
\endminipage
%
% 
\minipage{0.49\textwidth}
  \includegraphics[width=\linewidth]{figures/defense/defense_optimization.pdf}
\endminipage
%
% I don't understand the fooling rate on the right. The axis seems ot be just the number of queries.
% got it, so add % on the right axis works?
% Are the bars plotting the number of queries or the fooling rate? There are two axes but it's not clear what's being shown here.
% Darn yes, FR is only for the FR bars. Urm , let me find some technology to plot this correctly
%
\caption{\textbf{Effectiveness of our defense in efficient deep learning scenarios.} We show how much our defense reduces adversarial vulnerability. On the left, we show the RFRs we decrease in the transfer-based attacks. We show the query efficiency and the success on the right figure. \textbf{Base} is the undefended cases in Table~\ref{tbl:effectiveness-of-priors}, and \textbf{Ours} is the fine-tune last (FL) defense.}
%
\label{fig:defense_summary}
%
\end{figure*}

==> figures/similarity_comparison.tex <==


% Note
\begin{figure*}[h]
    % 
    \minipage{0.3\textwidth}
      \includegraphics[width=\linewidth]{figures/similarity.logits.box.png}
    \endminipage
    % 
    \hfill
    % 
    \minipage{0.3\textwidth}
      \includegraphics[width=\linewidth]{figures/similarity.gradients.box.png}
    \endminipage
    %
    \hfill
    %
    \minipage{0.38\textwidth}%
      %
      \centering
      \adjustbox{max width=\textwidth}{
        \begin{tabular}{@{}l|cc|cc|Sc@{}}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model $g$}}} & \multicolumn{2}{c|}{\textbf{Similarity}} & \multicolumn{2}{c|}{\textbf{Vuln. (Trans)}} & \multicolumn{2}{c}{\textbf{Vuln. (Optim.)}} \\ \cmidrule{2-7}
        %
         & \textbf{Out.} & \textbf{In.} & \textbf{FGSM} & \textbf{PGD} & \textbf{\# Q} & \textbf{FR} \\ \midrule \midrule
        %
        R50 (as-is) & 1.00 & 1.00 & 1.00 & 1.00 & 14.1 & 100\% \\
        R50 (a new) & 0.87 & 0.15 & 0.25 & 0.91 & 274.4 & 95\% \\ \midrule
        %
        % R50 (Q) & 1.00 & 0.61 & 1.00 & 1.00 & 14.1 & 100\% \\
        % R50 (P) & 0.89 & 0.33 & 0.89 & 1.00 & 19.5 & 100\% \\
        % R18 (KD) & 0.84 & 0.17 & 0.24 & 0.86 & 381.1 & 93\% \\
        % NAS & 0.82 & 0.14 & 0.13 & 0.76 & 979.3 & 80\% \\
        % MobileV2 & 0.81 & 0.14 & 0.24 & 0.76 & 580.3 & 89\% \\
        % Squeeze & 0.83 & 0.14 & 0.09 & 0.47 & 1547.1 & 67\% \\ \bottomrule
        % 
        % (The above is average, and the below is median; I take the median)
        R50 (Q) & 1.00 & 0.99 & 1.00 & 1.00 & 14.1 & 100\% \\
        R50 (P) & 0.97 & 0.41 & 0.89 & 1.00 & 19.5 & 100\% \\
        R18 (KD) & 0.94 & 0.08 & 0.24 & 0.86 & 381.1 & 93\% \\
        NAS & 0.87 & 0.14 & 0.05 & 0.76 & 979.3 & 80\% \\
        MobileV2 & 0.95 & 0.04 & 0.24 & 0.76 & 580.3 & 89\% \\
        Squeeze & 0.92 & 0.02 & 0.09 & 0.47 & 1547.1 & 67\% \\ \bottomrule
        %
        \end{tabular}
      }
      %
    \endminipage
    % 
    % \npc{Y axis might be eaiser to read as "similarity to resnet-50 model" or something like that.}\npc{Why no data on RN50 left plot?}
    % <- Update the Y-axis and I just excluded the baseline where the similarity is 1.0, RN from scratch is in third column.
    \caption{\textbf{Our similarity metrics accurately predicts the vulnerability to black-box adversarial examples.} We measure the similarities between the target (ResNet50) and the on-device models from Table~\ref{tbl:effectiveness-of-priors} at the outputs (left) and the input-gradients (middle) on CIFAR-10. We compare them with the vulnerability to the black-box adversarial attacks in the right table.}
    % 
    % {\color{red} These plots are not good; there are overlapping plots and it's not entirely clear what each plot means. Also, the feature space metrics are brittle, when there is permutations of elements. Plus, it would be better to measure the logits of the adversarial perturbations (FGSM, one-step only).}
    \label{fig:similarities}
    %
\end{figure*}

==> figures/trans_lu_v1.tex <==


\begin{figure}[h]
    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v1_0.01.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{0.01}}
    \endminipage
    %
    \hfill
    %
    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v1_0.1.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{0.1}}
    \endminipage
    %
    \hfill
    %
    \minipage{0.32\textwidth}%
      \includegraphics[width=\linewidth]{figures/trans_lu_v1_1.0.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{1.0}}
    \endminipage
    % 
    \caption{\textbf{Impact of the hyper-parameter choices in Eqn.~\ref{v1} on adversarial transferability (re-training).} We illustrate the accuracy of the model $f_s$ and the transferability of PGD-10 and FGSM attacks in different hyper-parameter ($\lambda$, $\alpha$) choices. Each plot is for $\lambda$ 0.01, 0.1, and 1.0, respectively. In each plot, we vary $\alpha$ in $\{1, 5, 10, 20, 30, 40, 50\}$. We re-train $f$ for constructing $f_s$.}
    \label{fig:trans_lu_v1}
    %
\end{figure}

==> figures/trans_lu_v1_scratch.tex <==



\begin{figure}[h]
    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v1_0.01_scratch.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{0.01}}
    \endminipage
    %
    \hfill
    %
    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v1_0.1_scratch.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{0.1}}
    \endminipage
    %
    \hfill
    %
    \minipage{0.32\textwidth}%
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{Nope.}}
    \endminipage
    % 
    \caption{\textbf{Impact of the hyper-parameter choices in Eqn.~\ref{v1} on adversarial transferability (training from scratch).} We illustrate the accuracy of the model $f_s$ and the transferability of PGD-10 and FGSM attacks in different hyper-parameter ($\lambda$, $\alpha$) choices. Each plot is for $\lambda$ 0.01 and 0.1, respectively. In each plot, we vary $\alpha$ in $\{1, 5, 10, 20, 30, 40, 50\}$. Here, we train $f_s$ from scratch.}
    \label{fig:trans_lu_v1}
    %
\end{figure}

==> figures/trans_lu_v2.tex <==


\begin{figure}[h]
    \centering
    % 
    \minipage{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v2.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{Use a pre-trained model)}}
    \endminipage
    %
    \minipage{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v2_scratch.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{Training from scratch}}
    \endminipage
    % 
    \caption{\textbf{Impact of the hyper-parameter choices in Eqn.~\ref{v2} on adversarial transferability.} We illustrate the accuracy of the model $f_s$ and the transferability of PGD-10 and FGSM attacks in different $\lambda$ choices. Each plot corresponds to a scenario: re-training (left) and training from scratch (right). We vary $\alpha$ in $\{0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.01, 0.1, 1.0\}$.}
    \label{fig:trans_lu_v2}
    %
\end{figure}

==> figures/trans_lu_v4.tex <==


\begin{figure}[h]
    \centering
    % 
    \minipage{0.45\textwidth}
      \includegraphics[width=\linewidth]{figures/trans_lu_v4.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{Use a pre-trained model)}}
    \endminipage
    %
    \minipage{0.45\textwidth}
    %   \includegraphics[width=\linewidth]{figures/trans_lu_v4_scratch.pdf}
      %
      \captionsetup{labelformat=empty}
      \caption{\textbf{Training from scratch (Yet).}}
    \endminipage
    % 
    \caption{\textbf{Impact of the hyper-parameter choices in Eqn.~\ref{v4} on adversarial transferability.} We illustrate the accuracy of the model $f_s$ and the transferability of PGD-10 and FGSM attacks in different $\lambda$ choices. Each plot corresponds to a scenario: re-training (left) and training from scratch (right). We vary $\alpha$ in $\{0.0001, 0.01, 0.1, 1.0\}$.}
    \label{fig:trans_lu_v2}
    %
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/baseline.tex <==



\begin{table}[h]
\centering
%
\adjustbox{max width=\linewidth}{
    \begin{tabular}{@{}cccc|cccc|cccc|cccc@{}}
    \toprule
    %
    \multicolumn{8}{c|}{\textbf{FGSM}} & \multicolumn{8}{c}{\textbf{PGD-20}} \\ \cmidrule{1-8} \cmidrule{9-16}
    %
    \multicolumn{4}{c|}{\textbf{FP32 $\rightarrow$ FP32}} & \multicolumn{4}{c|}{\textbf{Q8 $\rightarrow$ Q8}} & \multicolumn{4}{c|}{\textbf{FP32 $\rightarrow$ FP32}} & \multicolumn{4}{c}{\textbf{Q8 $\rightarrow$ Q8}} \\ \midrule \midrule
    %
    \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} \\
    %
    \textbf{A} & \textbf{25.9\%} & 71.5\% & 72.6\% & \textbf{A} & \textbf{25.8\%} & 71.4\% & 72.4\% & \textbf{A} & \textbf{0.0\%} & 11.2\% & 11.2\% & \textbf{A} & \textbf{0.0\%} & 11.2\% & 11.1\% \\
    %
    \textbf{B} & 70.3\% & \textbf{28.5\%} & 71.8\% & \textbf{B} & 70.3\% & \textbf{28.5\%} & 71.9\% & \textbf{B} & 7.0\% & \textbf{0.0\%} & 7.4\% & \textbf{B} & 7.1\% & \textbf{0.0\%} & 7.4\% \\
    %
    \textbf{C} & 69.7\% & 70.1\% & \textbf{29.0\%} & \textbf{C} & 69.7\% & 70.2\% & \textbf{28.9\%} & \textbf{C} & 6.2\% & 7.2\% & \textbf{0.0\%} & \textbf{C} & 6.3\% & 7.1\% & \textbf{0.0\%} \\ \bottomrule
    %
    \end{tabular}
}
%
\caption{\textbf{Transferability between CIFAR10 ResNet18 models with the same representation.}}
\label{tbl:baseline}
%
\end{table}

==> tables/network_depths.tex <==

% depths...
\begin{table*}[t]
%
\centering
%
\adjustbox{max width=\textwidth}{%
    %
    \begin{tabular}{@{}C{0.8cm}|ccccc|ccccc|ccccc@{}}
        \toprule
        %
        \multicolumn{16}{c}{\textbf{CIFAR10 ResNets}} \\ \midrule
         & \multicolumn{5}{c|}{\textbf{Clean}} & \multicolumn{5}{c|}{\textbf{FGSM}} & \multicolumn{5}{c}{\textbf{PGD-20}} \\ \midrule
        %
         & \textbf{18} & \textbf{34} & \textbf{50} & \textbf{101} & \textbf{152} & \textbf{18} & \textbf{34} & \textbf{50} & \textbf{101} & \textbf{152} & \textbf{18} & \textbf{34} & \textbf{50} & \textbf{101} & \textbf{152} \\ \midrule \midrule
        %
        \textbf{18} & 89.6\% & - & - & - & - & 19.0\% & 77.0\% & 77.4\% & 80.1\% & 79.6\% & \enspace0.0\% & 18.0\% & 16.3\% & 22.7\% & 21.4\% \\
        \textbf{34} & - & 91.0\% & - & - & - & 73.0\% & 23.8\% & 77.7\% & 78.6\% & 79.1\% & 17.2\% & \enspace0.0\% & 20.6\% & 22.4\% & 24.6\% \\
        \textbf{50} & - & - & 91.5\%& - & - & 71.4\% & 75.4\% & 27.3\% & 76.1\% & 76.0\% & 10.2\% & 13.4\% & \enspace0.0\% & 11.7\% & 10.2\% \\
        \textbf{101} & - & - & - & 92.5\% & - & 71.8\% & 74.2\% & 74.4\% & 30.9\% & 74.8\% & 11.7\% & 11.0\% & \enspace8.3\% & \enspace0.0\% & \enspace8.6\% \\
        \textbf{152} & - & - & - & - & 92.4\% & 71.0\% & 74.8\% & 72.9\% & 74.7\% & 31.4\% & 10.2\% & 12.5\% & \enspace6.8\% & \enspace7.7\% & \enspace0.0\% \\ \bottomrule
        %
    \end{tabular}
    %
}
%
\caption{\textbf{Cross-architecture transferability of adversarial examples.}
    We craft adversarial examples on five different ResNet models trained on CIFAR10. During training, we use the same hyper-parameters, \textit{e.g.}, the batch-size, the number of iterations, or the learning rate, for all the models. We use the entire test-set samples in CIFAR10 for crafting and measure the classification accuracy. We use the attack hyper-parameters ($\epsilon$, $\alpha$) = (0.03, 0.01). Each (row, col) is a (surrogate, victim) pair.
}
%
\end{table*}

% done.

==> tables/quantization.tex <==


\begin{table}[h]
\centering
%
\adjustbox{max width=\linewidth}{
    \begin{tabular}{@{}cccc|cccc|cccc|cccc@{}}
    \toprule
    %
    \multicolumn{8}{c|}{\textbf{FGSM}} & \multicolumn{8}{c}{\textbf{PGD-20}} \\ \cmidrule{1-8} \cmidrule{9-16}
    %
    \multicolumn{4}{c|}{\textbf{Q8 $\rightarrow$ FP32}} & \multicolumn{4}{c|}{\textbf{FP32 $\rightarrow$ Q8}} & \multicolumn{4}{c|}{\textbf{Q8 $\rightarrow$ FP32}} & \multicolumn{4}{c}{\textbf{FP32 $\rightarrow$ Q8}} \\ \midrule \midrule
    %
    \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{} & \textbf{A} & \textbf{B} & \textbf{C} \\
    %
    \textbf{A} & 25.9\% & {\color{blue} 72.4\%} & {\color{red} 72.4\%} & \textbf{A} & {\color{blue} 25.9\%} & {\color{blue} 71.5\%} & 72.4\% & \textbf{A} & 0.0\% & 11.2\% & {\color{red} 11.0\%} & \textbf{A} & 0.0\% & 11.2\% & {\color{blue} 11.3\%} \\
    %
    \textbf{B} & {\color{red} 70.1\%} & 28.5\% & {\color{blue} 71.9\%} & \textbf{B} & {\color{red} 70.2\%} & 28.5\% & {\color{red} 71.6\%} & \textbf{B} & 7.0\% & 0.0\% & 7.4\% & \textbf{B} & 7.1\% & 0.0\% & {\color{blue} 7.5\%} \\
    %
    \textbf{C} & 69.7\% & {\color{blue} 70.2\%} & {\color{red} 28.9\%} & \textbf{C} & {\color{red} 69.6\%} & {\color{red} 70.1\%} & {\color{blue} 29.0\%} & \textbf{C} & {\color{blue} 6.3\%} & {\color{red} 7.1\%} & 0.0\% & \textbf{C} & {\color{red} 6.2\%} & {\color{blue} 7.2\%} & 0.0\% \\ \bottomrule
    %
    \end{tabular}
}
%
\caption{\textbf{Transferability between CIFAR10 ResNet18 models with different representation.}}
\label{tbl:quantization}
%
\end{table}

==> tables/same-inputs.tex <==


% same input case
\begin{table*}[t]
%
\centering
%
\adjustbox{max width=\textwidth}{%
    %
    \begin{tabular}{@{}C{1.5cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}@{}}
        \toprule
        %
         & \multicolumn{2}{c|}{\textbf{Models (S: C10, V: C100)}} & \multicolumn{2}{c|}{\textbf{Models (S: C100, V: C10)}} & \multicolumn{2}{c}{\textbf{Ref. (White-box)}} \\ \midrule
        %
        \textbf{Cases} & \textbf{Base: $\mathcal{D}_{c10}$} & \textbf{Base: $\mathcal{D}_{c100}$} & \textbf{Base: $\mathcal{D}_{c10}$} & \textbf{Base: $\mathcal{D}_{c100}$} & \textbf{C10} & \textbf{C100} \\ \midrule \midrule
        %%
        \textbf{Clean} & 100.\%$^\dagger$ & \multirow{3}{*}{\textbf{N/A}} & \multirow{3}{*}{\textbf{N/A}} & 100.\%$^\dagger$ & 93.0\% & 72.3\% \\
        \textbf{FGSM} & 60.2\%$^\dagger$ &  &  & 73.4\%$^\dagger$ & 25.9\% & 12.0\% \\
        \textbf{PGD-20} & 26.7\%$^\dagger$ &  &  & 42.3\%$^\dagger$ & \enspace0.6\% & \enspace0.0\% \\ \bottomrule
        %
    \end{tabular}
}
%
\caption{\textbf{Cross-domain transferability of adversarial examples between two tasks sharing the same inputs.} 
    The left four columns show the transferability results. We craft adversarial examples on the surrogate models (\textbf{S}) and use them to attack the victim model (\textbf{V}). The second row includes the test datasets used for crafting adversarial examples. We use the entire test-set samples and measure the classification accuracy. We use the attack hyper-parameters ($\epsilon$, $\alpha$) = (0.03, 0.01). For reference, we provide the results from conventional white-box attacks. As we do not have the label conversion from C10 to C100, we use the pseudo-labels---the predictions of the other from a victim.
}
%
\end{table*}

% done.

==> tables/same-labels.tex <==

% same label case
\begin{table*}[ht]
%
\centering
%
\adjustbox{max width=\textwidth}{%
    %
    \begin{tabular}{@{}C{1.5cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}@{}}
        \toprule
        %
         & \multicolumn{2}{c|}{\textbf{Models (S: USPS, V: MNIST)}} & \multicolumn{2}{c|}{\textbf{Models (S: MNIST, V: USPS)}} & \multicolumn{2}{c}{\textbf{Ref. (White-box)}} \\ \midrule
        %
        \textbf{Cases} & \textbf{Base: $\mathcal{D}_{usps}$} & \textbf{Base: $\mathcal{D}_{mnist}$} & \textbf{Base: $\mathcal{D}_{usps}$} & \textbf{Base: $\mathcal{D}_{mnist}$} & \textbf{USPS} & \textbf{MNIST} \\ \midrule \midrule
        %%
        \textbf{Clean} & 92.3\% & 99.1\% & 97.7\% & 90.4\% & 97.7\% & 99.2\% \\
        \textbf{FGSM} & 91.7\% & 99.0\% & 97.3\% & 89.9\% & 95.8\% & 98.7\% \\
        \textbf{PGD-20} & 36.7\% & 85.9\% & 43.7\% & 47.7\% & \enspace0.2\% & \enspace6.3\% \\ \bottomrule
        %
    \end{tabular}
}
%
\caption{\textbf{Cross-domain transferability of adversarial examples between two tasks sharing the same labels.} 
    The left four columns show the transferability results. We craft adversarial examples on the surrogate models (\textbf{S}) and use them to attack the victim model (\textbf{V}). The second row includes the test datasets used for crafting adversarial examples. We use the entire test-set samples and measure the classification accuracy. We use the attack hyper-parameters ($\epsilon$, $\alpha$) = (0.3, 0.01). For reference, we provide the results from conventional white-box attacks. All the images are 28$\times$28-pixels.
}
%
\end{table*}

% done.
